A Relaxation Approach to Feature Selection for Linear Mixed Effects Models

Linear Mixed-Effects (LME) models are a fundamental tool for modeling correlated data, including cohort studies, longitudinal data analysis, and meta-analysis. Design and analysis of variable selection methods for LMEs is more difficult than for linear regression because LME models are nonlinear. In this work we propose a relaxation strategy and optimization methods that enable a wide range of variable selection methods for LMEs using both convex and nonconvex regularizers, including $\ell_1$, Adaptive-$\ell_1$, CAD, and $\ell_0$. The computational framework only requires the proximal operator for each regularizer to be available, and the implementation is available in an open source python package pysr3, consistent with the sklearn standard. The numerical results on simulated data sets indicate that the proposed strategy improves on the state of the art for both accuracy and compute time. The variable selection techniques are also validated on a real example using a data set on bullying victimization.

==> math_macros-jim2.tex <==
% derivatives
\newcommand{\dderiv}[2]{\frac{\mathrm{d}}{\mathrm{d}#2} (#1)}

% partial derivatives
\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand*{\pd}[3][]{\ensuremath{\frac{\partial^{#1} #2}{\partial #3}}}

% Integral dx
\newcommand{\dx}{\mathrm{d}x}

% Evaluation operator
\newcommand*{\at}[2]{\Big|_{#1}^{#2}}

% Probability macros
% Variance
\newcommand{\Var}{\mathrm{Var}}
% Covariance
\newcommand{\Cov}{\mathrm{Cov}}
% Bias
\newcommand{\Bias}{\mathrm{Bias}}
% Probability
\newcommand*{\prob}[1]{\ensuremath{\mathbb{P}\left[#1\right]}}
\newcommand*{\expectation}[1]{\ensuremath{\mathbb{E}\left[#1\right]}}
\newcommand*{\variance}[1]{\ensuremath{\mathbb{V}\left[#1\right]}}
% Indicator function of an event
\newcommand*{\ind}[1]{\ensuremath{\mathds{I}_{\left[#1\right]}}}

% Optimization macros
\DeclareMathOperator{\dom}{\mathrm{dom}}
\newcommand{\Diag}[1]{\mathrm{Diag}\left(#1\right)}
\newcommand{\diag}[1]{\mathrm{diag}\left(#1\right)}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\clco}{\overline{\conv}}
\newcommand{\gammax}{{\gam_{\mbox{\tiny max}}}}
\def\prox{{\mathrm{prox}}}
\DeclareMathOperator*{\proj}{\mathrm{Proj}}
\DeclareMathOperator*{\sign}{\mathrm{sign}}
\DeclareMathOperator*{\argmax}{\mathrm{argmax}}
\DeclareMathOperator*{\argmin}{\mathrm{argmin}}
\newcommand{\intr}[1]{\mathrm{int}\left( #1\right)}

\newcommand*{\pdef}{\ensuremath{\mathbb{S}_{++}}}
\newcommand*{\psdef}{\ensuremath{\mathbb{S}_{+}}}

%% \mathbb symbols
\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\A}{\mathbb{A}}
\DeclareMathOperator{\B}{\mathbb{B}}
\DeclareMathOperator{\R}{\mathbb{R}}
\DeclareMathOperator{\C}{\mathbb{C}}
\DeclareMathOperator{\X}{\mathbb{X}}
\DeclareMathOperator{\N}{\mathbb{N}}
\DeclareMathOperator{\Q}{\mathbb{Q}}
\DeclareMathOperator{\V}{\mathbb{V}}
\DeclareMathOperator{\bS}{\mathbb{S}}

%% \mathcal symbols
\DeclareMathOperator{\RR}{\mathcal{R}}
\DeclareMathOperator{\PP}{\mathcal{P}}
\DeclareMathOperator{\NN}{\mathcal{N}}
\def\CC{\mathcal{C}}
\DeclareMathOperator{\FF}{\mathcal{F}}
\DeclareMathOperator{\YY}{\mathcal{Y}}
\DeclareMathOperator{\XX}{\mathcal{X}}
\DeclareMathOperator{\LL}{\mathcal{L}}
\DeclareMathOperator{\wLL}{\widehat\LL}
\DeclareMathOperator{\OO}{\mathcal{O}}
\DeclareMathOperator{\II}{\mathcal{I}}
\def\TT{\mathcal{T}}
\def\hTT{{\widehat\TT}}
\def\SS{\mathcal{S}}
\def\hSS{{\widehat\SS}}
\DeclareMathOperator{\DD}{\mathcal{D}}
\DeclareMathOperator{\BB}{\mathcal{B}}
\def\MM{\mathcal{M}}
\def\uball{\mathbb{B}}
%\def\S{\mathcal{S}}

%% \tilde symbols
\newcommand{\tbeta}{\tilde\beta}
\newcommand{\tgamma}{\tilde\gamma}
\newcommand{\tu}{\tilde{u}}
\newcommand{\tr}{\tilde{r}}

%% \hat symbols
\newcommand{\hbeta}{\hat{\beta}}
\newcommand{\hgamma}{\hat{\gamma}}
\newcommand{\hxi}{\hat{\xi}}
\def\hy{\hat y}
\def\hX{\widehat X}

%% \bar symbols
\newcommand{\bmu}{\bar{\mu}}
\newcommand{\bgam}{\bar{\gamma}}


% limit arrow "goes to"
\newcommand{\goto}{\rightarrow}
%\newcommand{\gotowith}[2]{\xrightarrow[#2]{#1}}

% text above math symbol
%\newcommand{\textabove}[2]{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny #1}}}{#2}}}

% Big O
\newcommand{\bigo}{{\mathcal O}}

% 1/2
\newcommand{\half}{\mbox{\small$\frac{1}{2}$}}
% 1/2
\newcommand{\halfof}[1]{\frac{#1}{2}}

% Real numbers
\newcommand\reals{{{\rm l} \kern -.15em {\rm R} }}

% Complex numbers
\newcommand\complex{{\raisebox{.043ex}{\rule{0.07em}{1.56ex}} \hskip -.35em {\rm C}}}

% Matrix functions
\DeclareMathOperator{\trace}{Tr}

% Epigraphs
\DeclareMathOperator{\epi}{epi}

% matrix environment for vectors or matrices where elements are centered
\newenvironment{mat}{\left[\begin{array}{ccccccccccccccc}}{\end{array}\right]}
\newcommand\bcm{\begin{mat}}
\newcommand\ecm{\end{mat}}

% matrix environment for vectors or matrices where elements are right justified
\newenvironment{rmat}{\left[\begin{array}{rrrrrrrrrrrrr}}{\end{array}\right]}
\newcommand\brm{\begin{rmat}}
\newcommand\erm{\end{rmat}}

% for left brace and a set of choices
\newenvironment{choices}{\left\{ \begin{array}{ll}}{\end{array}\right.}
\newcommand\when{&\text{if~}}
\newcommand\otherwise{&\text{otherwise}}
% sample usage:
%  \delta_{ij} = \begin{choices} 1 \when i=j, \\ 0 \otherwise \end{choices}

% For equations: first argument is a label, second is the equation 
\newcommand{\eql}[2]{\begin{equation}\label{eq:#1}\begin{split}#2\end{split}\end{equation}}
% Or just the equation 
\newcommand{\eq}[1]{\begin{equation}\begin{split}#1\end{split}\end{equation}}

% some useful macros for finite difference methods:
\newcommand\unp{U^{n+1}}
\newcommand\unm{U^{n-1}}
\newcommand\un{U^{n}}

% paired parenthesis
%\DeclarePairedDelimiter\pa{(}{)}%
%\DeclarePairedDelimiter\bra{[}{]}%
%\DeclarePairedDelimiter\curly{\{}{\}}%
%\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
%\DeclarePairedDelimiter\norm{\lVert}{\rVert}%
%\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}%
%\DeclarePairedDelimiter\ceil{\lceil}{\rceil}%

% Theorems and co. environments setup
\newtheorem{definition}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}{Remark}

% colorful box (for putting around equality signs etc)
%\newtcbox{\mywboxtext}[1]{on line,colback=white,colframe=#1,size=fbox,arc=3pt,boxrule=0.8pt}
%\newcommand{\boxaround}[2]{\mywboxtext{#2}{$#1$}}

% A few things for Jim
\def\bW{{\mathbb{W}}}
\def\Rn{{\R^n}}
\def\eR{{\overline\R}}
\def\Rp{{\R^p}}
\def\Rq{{\R^q}}
\def\Rm{{\R^m}}
\def\hf{{\hat f}}
\def\hy{{\hat y}}
\def\hr{{\hat r}}
\def\hR{{\widehat R}}
\def\tR{{\widetilde R}}
\def\hs{{\hat s}}
\def\bv{{\bar v}}
\def\tx{{\tilde x}}
\def\ty{{\tilde y}}
\def\tw{{\tilde w}}
\def\br{{\bar r}}
\def\bu{{\bar u}}
\def\hZ{{\widehat Z}}
\def\tK{{\widetilde K}}
\def\wG{{\widehat G}}
\def\one{\mathbf{1}}
\def\zero{\mathbf{0}}
\def\lam{\lambda}
\def\blam{{\bar\lambda}}
\def\lamb{\lambda_b}
\def\lamg{\lambda_g}
\def\Lam{\Lambda}
\def\alf{\alpha}
\def\talf{{\tilde\alpha}}
\def\tkappa{{\tilde\kappa}}
\def\balf{{\bar\alpha}}
\def\bgam{{\bar\gamma}}
\def\bbeta{{\bar\beta}}
\def\bbeta{{\bar\beta}}
\def\bxi{{\bar\xi}}
\def\bw{{\bar w}}
\def\hw{{\hat w}}
\def\bx{{\bar x}}
\def\by{{\bar y}}
\def\bz{{\bar z}}
\def\bv{{\bar v}}
\def\hv{{\hat v}}
\def\hx{{\hat x}}
\def\he{{\hat{\mathrm{e}}}}
\def\hp{{\hat{\mathrm{p}}}}
\def\tv{{\tilde v}}
\def\gam{\gamma}
\def\hgam{{\hat\gam}}
\def\tgam{{\tilde\gam}}
\def\bgam{{\bar\gam}}
\def\Gam{\Gamma}
\def\bOmega{{\overline\Omega}}
\def\bomega{{\bar\omega}}
\def\del{\delta}
\def\Del{\Delta}
\def\eps{\epsilon}
\newcommand{\lDel}{\mbox{\small$\Del$}}
\def\Sig{\Sigma}
\def\sig{\sigma}
\def\BB{{\mathcal{B}}}
\def\GG{{\mathcal{G}}}
\def\hGG{{\widehat\GG}}
\def\VV{{\mathcal{V}}}
\def\RR{{\mathcal{R}}}
\def\hRR{{\widehat\RR}}
\def\tLL{{\widetilde\LL}}
\def\hLL{{\widehat\LL_\mu}}
\def\hDD{{\widehat\DD}}
\def\Dfr{\mathfrak{D}}
\def\LLlam{{\LL_\lam}}
\def\hOmega{{\widehat\Omega}}
\def\mmax{\text{max}}
\def\mmin{\text{min}}
\newcommand\map[3]{#1:#2\rightarrow #3}
\def\Ran{\mathrm{Ran}\,}
\newcommand{\rset}[2]{\left\{#1\,\left|\,#2\right\}\right.}
\newcommand{\lset}[2]{\left\{#1\,\left|\,#2\right.\right\}}
\newcommand{\norm}[1]{\left\Vert #1\right\Vert}
\newcommand{\im}[1]{{\mathrm{Im}\left(#1\right)}}
\newcommand{\lev}[2]{{\mathrm{lev}_{#1}(#2)}}
\newcommand{\ip}[2]{\left\langle #1,\, #2\right\rangle}

\def\bgk{(\beta^k,\gam^k)}
\def\tbgk{(\tbeta^k,\tgam^k)}
\def\bg{(\beta,\gam)}
\def\tbg{(\tbeta,\tgam)}
\def\bbg{(\bar\beta,\bar\gam)}
\def\hbg{(\hat\beta,\hat\gam)}
\def\emu{{\eta,\mu}}
\def\phimu{\phi_\mu}
\def\umu{u_\mu}
\def\uemu{{u_{\eta,\mu}}}
\def\keta{\kappa_\eta}
\def\Rqp{\R^q_+}
\def\vphi{\varphi}
\def\vmu{v_\mu}
\def\xmu{x_\mu}

